WheaCha: A Method for Explaining the Predictions of Models of Code

Attribution methods have emerged as a popular approach to interpreting model predictions based on the relevance of input features. Although the feature importance ranking can provide insights of how models arrive at a prediction from a raw input, they do not give a clear-cut definition of the key features models use for the prediction. In this paper, we present a new method, called WheaCha, for explaining the predictions of code models. Although WheaCha employs the same mechanism of tracing model predictions back to the input features, it differs from all existing attribution methods in crucial ways. Specifically, WheaCha divides an input program into "wheat" (i.e., the defining features that are the reason for which models predict the label that they predict) and the rest "chaff" for any prediction of a learned code model. We realize WheaCha in a tool, HuoYan, and use it to explain four prominent code models: code2vec, seq-GNN, GGNN, and CodeBERT. Results show (1) HuoYan is efficient - taking on average under twenty seconds to compute the wheat for an input program in an end-to-end fashion (i.e., including model prediction time); (2) the wheat that all models use to predict input programs is made of simple syntactic or even lexical properties (i.e., identifier names); (3) Based on wheat, we present a novel approach to explaining the predictions of code models through the lens of training data.

==> comments.tex <==
\section{Comments}

\wyc{Here are my comments}

1.  Regarding `$(t_{n}^{\tilde{P}})_{n\in\mathbb{N}} = (t_{m_{k}}^{P})_{k\in\mathbb{N}}$ where $(m_k)_{k\in\mathbb{N}}$ is a strictly increasing sequence of positive integers.' The formula doesn't restrict $n$, it may indicate ($1,2,3,4,5$) is a subsequence of ($5,4,3,2,1$).

I think the following two may be better:

$(t_{n}^{\tilde{P}})_{n\in\mathbb{N}} = (t_{m_{k}}^{P})_{k\in\mathbb{N}}$ where $(m_k)$ and $(n)$ are strictly increasing sequences of positive integers. 

$(t_{k}^{\tilde{P}}) = (t_{m_{k}}^{P})_{k\in\mathbb{N}}$ where $(m_k)_{k\in\mathbb{N}}$ is a strictly increasing sequence of positive integers.


2. Regarding the proof of theorem 2.1, Is the following proof also ok (may reduce the space if it is ok)?

Because $P$ itself satisfies \textit{constituent}, \textit{sufficient}, and \textit{necessary} requirement in Definition~\ref{def:keyfea}. It has to be the \textit{minimal} requirement that $P$ violates. 
Because the domain that contains all sets of statements/expressions whose token sequence is a subsequence of $P$'s is finite, and the size of the candidate programs will monotonically decreases (\ie,
$\lvert (t_{n}^{P^\prime})_{n\in\mathbb{N}} \rvert < \lvert(t_{n}^{P})_{n\in\mathbb{N}}\rvert$, 
$\lvert (t_{n}^{P^{\prime\prime}})_{n\in\mathbb{N}} \rvert < \lvert(t_{n}^{P^{\prime}})_{n\in\mathbb{N}}\rvert$, and so on), there will be a global minimal set of statements/expressions $\tilde{P}$ that satisfies all requirements in Definition~\ref{def:keyfea}, which implies that $\tilde{P}$ is the defining features for $P$. This contradicts the assumption that $\tilde{P}$ does not exist for $P$.	

3. please double check my edits.

4. (1)  `However, they can compute the attributions for all input features in a single forward and backward pass through the network, \textbf{resulted} ( \textbf{resulting} ) in higher efficiency.'  (2) `We study code summarization models due to the tremendous impact they made \textbf{to} (on?) the programming language field.' (3) To sum up, an input feature’s satisfaction of the sufficient requirement does not give any indication \textbf{on} (of?) the necessity of the remaining features in the same input, thus the contradiction dissolves. (4) I change the only two occurrences of `defining feature' to `defining features'. (5) `we may only need to \textbf{retrain} (\textbf{retain}?) its syntactic structure without the specific identifier names.' (6) `finally \textit{RestoreNode} reverts a node \textbf{back} (remove \textbf{back}?) to the saved node.' (7) I changed `~\citet{szegedy2013intriguing} is the first' to `~\citet{szegedy2013intriguing} are the first to discover'. But didn't change `\citet{zeiler2011adaptive} \textbf{is} a typical example in the image classification domain. In particular, it \textbf{occludes} different segments of an input image and visualizes the change in the activation of later layers. ' (8) `The function \texttt{SelectionUtil} first creates a subset with the parameter \texttt{size}, ' The \texttt{size} here seems to be \texttt{k}. (9) I removed 'a' in  'a smaller defining features'.  (10) 'Surprisingly, the defining features that sequence GNN uses \textbf{is} the smallest while it is \textbf{the} supposedly the most expressive model that also utilizes semantic properties of input programs.' shall we change it to 'Surprisingly, the defining features that sequence GNN uses are the smallest while the model is supposedly the most expressive one that also utilizes semantic properties of input programs.' (11) `we exhaustively generate the test candidates for each method \textbf{before hand} (beforehand?) in a parallel fashion'



==> method.tex <==
\section{The Reduce and Mutate Method}
\label{sec:met}

In this section, we give a detailed presentation of \textit{Reduce} and \textit{Mutate} for identifying the defining features that code summarization models use for prediction. 


%In particular, we describe the two key functional components: \textit{Reduce} and \textit{Mutate}. 
%We also present an example use of the revealed key features.

\subsection{Reduce}
\label{subsec:red}

%A brute-force approach is to exhaust all subsets of the statements in the method. This yields an exponential time algorithm which would incur $2^{n}\!-\!2$ ($n$ is the number of statements in the method, and we don't need to consider the empty subset or the method itself, hence ``$-2$'') trials in the worst case. In principle, such an algorithm is unlikely to scale to methods of a large number of statements, however, based on our prior observation that few statements in a method already cover the defining features, the algorithm would quickly find the global minimal region as long as it traverses the regions in the ascending order of the size. 
%

Algorithm~\ref{alg:findregion} gives the functionality of the \textit{Reduce} step. The \texttt{for} loop at line~\ref{line:loop1} gradually increases the size of the subsets drawn from the list of flattened statements (line~\ref{line:flat}) while searching for the minimal code fragments. The function \texttt{SelectionUtil} first creates a subset with the parameter \texttt{k}, then invokes
%creates subsets of the size $k$, the induction variable of the aforementioned \texttt{for} loop, via recursion, and then pass 
\texttt{Verify}, another function that checks the validity of the created subset against the \textit{sufficient} and \textit{necessary} requirement. Once the created subset is found out to be valid, we add it to the collection of all minimal subsets \texttt{fragments} (line~\ref{line:addtoreg}). Below, we present the technical details about two functions: \texttt{Flatten} (line~\ref{line:flat}) and \texttt{Reconstruct} (line~\ref{line:recon}).

The goal of the \texttt{Flatten} function is to reduce an input method into a set of statements. Specifically, for a non-control statement such as declarations, assignments, or method calls, \texttt{Flatten} directly adds them to the set (line~\ref{line:flat:dadd}); for a control statement such as \texttt{if} statement or \texttt{while} loop, \texttt{Flatten} first adds the predicate of the control statement (\eg, \texttt{if} \texttt{(}condition\texttt{)}) with an empty body 
%and the associated block if present (\eg, \texttt{while} \texttt{(}condition\texttt{)}\{ \}) 
as a separate statement to the set (line~\ref{line:flat:addctlstmt});
%\footnote{Note that block has to be directly associated with the predicate of a control statement. This is the reason we separate the block from the case label in Figure~\ref{fig:handleFea} since it is not associated with the \texttt{switch} predicate.}; 
and then in order to process statements in their body, we recursively call function \texttt{Flatten} with the body of the control statement as the function argument  (line~\ref{line:flat:rec}). The function terminates when we completely flatten the input program. Note that we bind certain code structures as a single statement to ensure the syntactic validity of the added statements. For example, \texttt{case} or \texttt{default} labels will be automatically added with the \texttt{switch} predicate whenever a \texttt{switch} statement is flattened. 
%Finally, \texttt{Flatten} adds the entire parameter list of an input method as another statement.


\begin{algorithm}[!tbp]

	\algnewcommand\Sz{size\xspace}
	\algnewcommand\Md{method\xspace}
	\algnewcommand\Mn{method.name\xspace}		
	\algnewcommand\Mb{method.body\xspace}	
	\algnewcommand\Mp{method.parameters\xspace}	
	\algnewcommand\Mh{method.head\xspace}	
	\algnewcommand\Mr{method\_header\xspace}		
	\algnewcommand\Sd{new\xspace}	
	\algnewcommand\Sr{new Method(remaining\_statements, method.head)\xspace}		
	\algnewcommand\Ml{model\xspace}
	\algnewcommand\Lb{label\xspace}
	\algnewcommand\Pd{result\xspace}	
	\algnewcommand\K{k\xspace}
	\algnewcommand\I{i\xspace}
	\algnewcommand\S{s\xspace}
	\algnewcommand\St{selected\_statements\xspace}		
	\algnewcommand\Rs{remaining\_statements\xspace}
	\algnewcommand\Ts{statements\xspace}
	\algnewcommand\Ti{statements[i]\xspace}	
	\algnewcommand\Tz{statements.size\xspace}
	\algnewcommand\To{statements.size-1\xspace}		
	\algnewcommand\Tr{traversed\_statements\xspace}
	\algnewcommand\Se{fragment\xspace}	
	\algnewcommand\Rm{region[-1]\xspace}	
	\algnewcommand\Mm{m\xspace}
	\algnewcommand\Ic{is\_continue\xspace}
	\algnewcommand\Nm{m\xspace}
	\algnewcommand\Ci{index\xspace}
	\algnewcommand\Cd{depth\xspace}
	\algnewcommand\Ip{index++\xspace}
	\algnewcommand\Dp{depth++\xspace}
	\algnewcommand\Me{max\_depth\xspace}
	\algnewcommand\Sa{selected\xspace}			
	\algnewcommand\Lz{selected.size\xspace}
	\algnewcommand\rec{Reconstruct\xspace}
	\algnewcommand\vef{Verify\xspace}
	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

	\caption{Find the minimal fragment of code in a method.}
	\label{alg:findregion}
 \begin{algorithmic}[1]
\Procedure{FindMinimalFragment}{$method, model$}
 \State statements $\gets$ \Call{Flatten}{method} \label{line:flat}
 \LineComment{\hspace{\algorithmicindent} \(\triangleright\)  traversing all subsets in the ascending of the cardinality; `-1' excludes the entire set.}
\For{k $\gets 1$  \textbf{to} statements.size - 1 \label{line:loop1}}
  %\State  region $\gets$ \Call{SelectionUtil}{statements, 0, 0, k, $\varnothing$, method, model}
  \State  fragments $\gets$ \Call{SelectionUtil}{statements, k, method, model}
\If{fragments $\neq$ $\varnothing$} \label{line:ifregion}
	\State  \Return{fragments} \label{line:retregion}
\EndIf 
\EndFor
\EndProcedure

\item[]


\Function{Flatten}{$\Md$}\label{line:flatten}
	\State stmts $\gets$ $\varnothing $
	\Foreach{stmt $\in$ $\Md$.statements}
    	\If {stmt \textbf{is} ControlStmt} \Comment{if \text{stmt} is a control statement}
    		\State stmts $\gets$ stmts $\cup$ stmt.predicate \label{line:flat:addctlstmt}
    		\State stmts $\gets$ stmts $\cup$ \Call{Flatten}{stmt.body} \label{line:flat:rec}
    	\Else
    		\State stmts $\gets$ stmts $\cup$ stmt \label{line:flat:dadd}
    	\EndIf
	\EndForeach
	\State  \Return{stmts}
\EndFunction


\item[]

\Function{SelectionUtil}{$\Ts, \K, \Md, \Ml$}
%    \LineComment{getting all possible combinations of statements.}
%  	 and returning regions satisfy \textit{sufficient} and \textit{necessary} requirements.}
    
	\State sets $\gets$ \textit{CombinationsOfKStatement}\! (\Ts, \K) \Comment{getting combinations of size {k}}
	\State fragments $\gets$ $\varnothing $
	\Foreach{set $\in$ sets}
			\State suff\_mth, nec\_mth $\gets$ \textit{\rec}\! (set, \Md)  \label{line:recon} %\Comment{returns two methods}
			\If{\textit{\vef}\! ({suff\_mth, nec\_mth, \Ml})} \Comment{check the validity of set} \label{line:verify}	
				\State fragments $\gets$ fragments $\cup$ set \label{line:addtoreg}	

			\EndIf						
	\EndForeach
	\State  \Return{fragments}
\EndFunction

%\Function{SelectionUtil}{$\Ts, \Ci, \Cd, \Me, \Se, \Md, \Ml$}
%\If{\Cd  $<$ \Me} 
%	\For{i $\gets$ \Ci  \textbf{to} \Tz \label{line:loop2}}
%		\State  \Se.\textit{Add}\! (\Ti)
%		\State  \Call{SelectionUtil}{\Ts, \Ip, \Dp, \Me, \Se, \Md, \Ml}\label{line:rec} 
%			\If{\Lz $=$ \Me} \Comment{ensure a subset is checked only once}
%			%\State \! s $\gets$ \textit{Verify}({\Ml, \Md, \Se}) \Comment{verifying \textit{sufficient} and \textit{necessary} requirement} \label{line:verify}
%			%\If{s}
%			\State nec\_mth, suff\_mth $\gets$ \textit{\rec(\Me, \Se)} \Comment{returns two methods} \label{line:recon} 
%			\If{\textit{\vef}\! ({nec\_mth, suff\_mth, \Md})} \Comment{check against \textit{sufficient} and \textit{necessary}} \label{line:verify}											 
%				\State	\Return{\textit{\Se}}
%			\EndIf
%		\EndIf
%		\State \Se.\textit{Remove}\! (\Rm) \Comment{remove the last statement}
%	\EndFor
%\EndIf 
%\EndFunction

%\item[]
%
%\Function{Verify}{$\Ml, \Md, \Se$}\label{line:verify}
%	\State \Mm $\gets$ \Sd \textit{Method}\! (\Md, \Se)  \label{line:region}
%	\State \Pd $\gets$ \Ml.\textit{Predict}\! (\Mm)\;
%	\If{\Pd $=$ \Mn} 								 
%		\State \!\!\Pd $\gets$ \Ml.\textit{Predict}\! (\Md\!$\setminus$\! \Se)\;\label{line:rem}
%		\If{\Pd $\neq$ \Mn} 
%			\State \Return{\textit{True}}
%		\EndIf
%	\EndIf
%	\State \Return{\textit{False}}
%\EndFunction
\end{algorithmic}
\end{algorithm}

%
%\begin{algorithm}[!tbp]
%	\SetKwInOut{Input}{input}
%	\SetKwInOut{Output}{output}
%	
%	\DontPrintSemicolon
%	\SetKwProg{myproc}{procedure}{}{}
%	\SetKwFunction{proc}{FindMinimalRegion}
%	\SetKwProg{myfunc}{function}{}{}
%	\SetKwFunction{procc}{SelectionUtil}
%	\SetKwFunction{proco}{Verify}
%	
%	\SetKwData{Sz}{size}
%	\SetKwData{Md}{method}
%	\SetKwData{Mn}{method.name}		
%	\SetKwData{Mb}{method.body}	
%	\SetKwData{Mp}{method.parameters}	
%	\SetKwData{Mh}{method.head}	
%	\SetKwData{Mr}{method\_header}		
%	\SetKwData{Sd}{new}	
%	\SetKwData{Sr}{new Method(remaining\_statements, method.head)}		
%	\SetKwData{Ml}{model}
%	\SetKwData{Lb}{label}
%	\SetKwData{Pd}{result}	
%	\SetKwData{K}{k}
%	\SetKwData{I}{i}
%	\SetKwData{S}{s}
%	\SetKwData{St}{selected\_statements}		
%	\SetKwData{Rs}{remaining\_statements}
%	\SetKwData{Ts}{statements}
%	\SetKwData{Ti}{statements[i]}	
%	\SetKwData{Tz}{statements.size}
%	\SetKwData{To}{statements.size-1}		
%	\SetKwData{Tr}{traversed\_statements}
%	\SetKwData{Se}{region}	
%	\SetKwData{Rm}{region[-1]}	
%	\SetKwData{Mm}{m}
%	\SetKwData{Ic}{is\_continue}
%	\SetKwData{Nm}{m}
%	\SetKwData{Ci}{index}
%	\SetKwData{Cd}{depth}
%	\SetKwData{Ip}{index++}
%	\SetKwData{Dp}{depth++}
%	\SetKwData{Me}{max\_depth}
%	\SetKwData{Sa}{selected}			
%	\SetKwData{Lz}{selected.size}			
%
%	\SetKw{Ot}{to}
%	
%	\Input{\Md, \Ml}
%	\Output{\Se}
%	\myproc{\proc{\Md, \Ml}}{ 
%		\Begin{
%			%\tcc{turning the method into a set of state- ments including control predicate, non- control statement, and parameters.}
%			\Ts $\gets$ \textit{Flatten}\! (\Md) \\\label{line:flat}
%			\tcc{traversing the subsets of statements in the ascending of the cardinality; `-1' excludes the entire set.}
%			\For{\K $\gets 1$ \Ot \To}{\label{line:loop1}
%				\Se $\gets$ \textit{SelectionUtil}\! (\Ts, 0, 0, \K, $\varnothing$, \Md, \Ml)\\
%				\If{\Se $\neq$ $\varnothing$} {
%					\Return{\Se}
%				}
%			}
%		}
%	}	
%	
%%	\tcp{recursively calling itself to form a subset.}			
%	\myfunc{\procc{\Ts, \Ci, \Cd, \Me, \Se, \Md, \Ml}}{ 
%		\Begin{
%			\If{\Cd $<$ \Me} {
%				\For{\I $\gets$ \Ci \Ot \Tz}{\label{line:loop2}
%					\Se.\textit{Add}\! (\Ti) \\
%					\textit{SelectionUtil}\! (\Ts, \Ip, \Dp, \Me, \Se, \Md, \Ml) \\\label{line:rec}
%					\tcc{the following if condition prevents a subset from being checked more than once}%with different value of max\_depth
%					%					\eg, a subset of one element will be checked when max\_depth equals to 1; the very same subset will be checked again when max\_depth equals to 2 after all its supersets of size two have been checked.
%					\If{\Lz $=$ \Me} {
%						\!\S $\gets$ \textit{Verify}\! (\Ml, \Md, \Se)
%						\If{\S} {										 
%							\Return{\textit{\Se}}
%						}						
%					}
%					\tcp{remove the last statement}
%					\Se.\textit{Remove}\! (\Rm)
%				}
%			}
%			\Return{$\varnothing$}
%		}
%	}
%	
%%	\tcp{verifying a subset against the requirements.}			
%	\myfunc{\proco{\Ml, \Md, \Se}}{\label{line:verify}
%		\Begin{
%			\Mm $\gets$ \Sd \textit{Method}\! (\Md, \Se)  \\\label{line:region}
%			
%			\Pd $\gets$ \Ml.\textit{Predict}\! (\Mm)\;
%			
%			\If{\Pd $=$ \Mn} {										 
%				\!\!\Pd $\gets$ \Ml.\textit{Predict}\! (\Md\!$\setminus$\! \Se)\;\label{line:rem}
%				\If{\Pd $\neq$ \Mn} {
%					\Return{\textit{True}}
%				}
%			}
%			\Return{\textit{False}}		
%		}
%	}
%	\caption{Find the minimal region in a method.\ke{add the implementation for Flatten; whole algorithm should fit in one page}}
%	\label{alg:findregion}
%\end{algorithm}

%As for the \texttt{Verify} function, we discuss the constitution of the new method based on the minimal set of statements (line~\ref{line:region}) and define the \textit{subtraction} operation performed for checking the \textit{necessary} requirement (line~\ref{line:rem}). Regarding the creation of the new method, first, it retains the return type of the original input; then, depending on whether or not the minimal set of statements contains the parameters of the input method, we either add them to its own parameter list or leave the list empty. Finally, we copy the remaining statements in the set to the body of the new method. Note that statements in the new method's body will always be listed in a sequential order no matter their relationship in the AST of the original input, for example, an assignment statement that was in a \texttt{for} loop will be moved outside as a separate statement in the new method's body. Given the constitution of the new method, the \textit{subtraction} operation naturally follows. Below we give the definition.
%As for the \texttt{Verify} function, we discuss the constitution of the new method based on the minimal set of statements and define the \textit{subtraction} operation performed for checking the \textit{necessary} requirement. Regarding the creation of the new method, first, it retains the return type of the original input; then, depending on whether or not the minimal set of statements contains the parameters of the input method, we either add them to its own parameter list or leave the list empty. Finally, we copy the remaining statements in the set to the body of the new method. Note that statements in the new method's body will always be listed in a sequential order no matter their relationship in the AST of the original input, for example, an assignment statement that was in a \texttt{for} loop will be moved outside as a separate statement in the new method's body. Given the constitution of the new method, the \textit{subtraction} operation naturally follows. Below we give the definition.
%
%\begin{definition}(\textit{Subtraction of Statements})\label{def:remv1}
%	Let $P$ be a method. Let $\tilde{P}$ be the set of statements that Algorithm~\ref{alg:findregion} discovers from $P$. $P \setminus \tilde{P}$ is defined to be $\forall S \in \tilde{P} \, P \setminus S$ where $P \setminus S$ is removing the entire subtree rooted at $\mathit{root}$($S$) from $P$'s AST if $S$ is a parameter list or a non-control statement ($\mathit{root}$($S$) returns the root of $S$'s AST); otherwise, $P \setminus S$ is removing $\mathit{root}$($S$), its child node denoting the predicate of $S$, and the other child node denoting the block if present, and making the remaining children of $\mathit{root}$($S$) or the block node as the children of $\mathit{root}$($S$)'s parent.
%\end{definition}
%\vspace{-3pt}

\texttt{Reconstruct} function (line~\ref{line:recon}) returns two new programs: one for verifying against the \textit{sufficient} requirement (\ie, \texttt{suff\_mth}) and the other for verifying against the \textit{necessary} requirement (\ie, \texttt{nec\_mth}).
Regarding the construction of \texttt{suff\_mth}, when the selected combination, denoted by \texttt{set}, contains only one element, we place the single statement inside the body of \textit{suff\_mth} while copying the method header from \texttt{method}, otherwise, we rearrange the statements in \texttt{set} to reflect the syntactic structure of the input method. For example, an assignment statement will be placed back into the body of a \texttt{for} loop if that was the syntactic structure the input method possesses originally. To construct \texttt{nec\_mth}, we simply subtract the statements in \texttt{set} from the original input \texttt{method} (Definition~\ref{def:subtra}).

% is constructed by assembling statements in $\textit{method}\setminus\textit{region}$ following the structure of \textit{method}. After the \texttt{Reconstruct} function, the algorithm add the \textit{region} to \textit{regions}  when  \textit{suff\_mth} and \textit{nec\_mth} satisfy the \textit{sufficient} and \textit{necessary} requirements, respectively (lines~\ref{line:verify} to ~\ref{line:addtoreg}).

\vspace*{3pt}
\noindent
\textbf{\textit{Minimality}}\, Algorithm~\ref{alg:findregion} traverses the subsets of $P$ in the ascending order of the cardinality while checking the validity of each subset against the two requirements, therefore, the first subset it finds is the smallest among all. Furthermore, Algorithm~\ref{alg:findregion} only collects the subsets that have the same size as the first subset it finds. Therefore, Algorithm~\ref{alg:findregion} always returns the minimal sets of statements that satisfy the two requirements.

%\vspace{-1pt}
%\begin{theorem}[Minimal Region]\label{the:miniR}
%	Let a method $P$ be a set of statements given as the input to Algorithm~\ref{alg:keyfea}.
%%	 (\eg, control predicates, non-control statements, and parameters). 
%The output, denoted by $R$, is the smallest subset of $P$ that satisfies the \textit{sufficient} and \textit{necessary} requirements (\ie, $\nexists S\subseteq P \, \lvert S \rvert < \lvert R \rvert$ and $S$ also satisfies the two requirements).
%\end{theorem}
%\vspace{-7pt}
%
%\begin{proof}
%	By design, Algorithm~\ref{alg:findregion} traverses the subsets of $P$ in the ascending order of the cardinality while checking the validity of each subset against the two requirements, therefore, the first subset it finds is the smallest among all. 
%\end{proof}
%\vspace{-3pt}

%\vspace*{3pt}
%\noindent
%\textbf{\textit{Time Complexity}}\, We analyze the running time of Algorithm~\ref{alg:findregion}.
%%We emphasize that our analysis takes into account the actual distribution of inputs, albeit
%In theory, the algorithm runs in exponential time. However, considering over eight hundred thousand test methods in Java-small, Java-med, and Java-large as the inputs, Algorithm~\ref{alg:findregion} runs in cubic time in the worst case because the size of the minimal code fragment never exceeds three for each of the evaluated models. Furthermore, since the minimal region of three statements rarely occurs, we argue the average-case complexity, which we analyze below, is a more accurate measure of Algorithm~\ref{alg:findregion}'s performance in practice. 
%
%We focus on the process of traversing the subsets of \texttt{statements}
%%(line~\ref{line:loop1},~\ref{line:loop2} and~\ref{line:rec}) 
%in Algorithm~\ref{alg:findregion} since the remaining steps take $O(1)$ time.
%%\footnote{Strictly speaking, model prediction time is not $O(1)$, nevertheless, it's an external source of time consumption, which is mostly independent to Algorithm~\ref{alg:findregion}. 
%%Therefore, we simplify it to be $O(1)$.}. 
%On average, the traversal takes $t_{ave}$ to execute:
%\vspace{-3pt}
%\begin{equation*} \label{eq:eq1}
%\begin{split}
%t_{ave} & = \sum_{k=0}^{\infty} p_k t(k) \\
%& = \sum_{k=0}^{\infty} p_k (k*t_{one}) = t_{one}\sum_{k=0}^{\infty} p_k k  \\
%%		& = O(1) \sum_{i=0}^{\infty} p_k k		
%\end{split}
%\end{equation*}\vspace{-1pt}where $t(k)$ denotes the average time taken to traverse $k$ subsets; and $p_k$ denotes the probability of an input causing $k$ subsets to be traversed. Since the average time taken to traverse one subset is independent of the total number of subsets Algorithm~\ref{alg:findregion} requires, we replace $t(k)$ with $k*t_{one}$ where $t_{one}$ is the average time taken to traverse one subset.
%
%Now, incorporating the distribution of our inputs:
%%\begin{equation} \label{eq:eq3}
%%\begin{split}
%%t_{one}\sum_{k=0}^{\infty} p_k k &= t_{one}\sum_{k=1}^{\lvert P \rvert^3} p_k k \, \text{(} p_k=0 \, \text{when} \, k=0 \, \text{or} \, k>\lvert P \rvert^3  \text{)}\\		
%%& < t_{one} (p_{\lvert P \rvert} \lvert P \rvert + 
%%p_{\lvert P \rvert^2} \lvert P \rvert^2 +
%%p_{\lvert P \rvert^3} \lvert P \rvert^3)
%%\end{split}
%%\end{equation}
%\begin{equation*} \label{eq:eq2}
%\begin{split}
%%t_{ave} & = t_{one}\sum_{k=0}^{\infty} p_k k \\
%t_{ave} & = t_{one}\sum_{k=1}^{\lvert P \rvert^3} p_k k \, \text{(} p_k=0 \, \text{when} \, k=0 \, \text{or} \, k>\lvert P \rvert^3  \text{)}\\		
%		& < t_{one} (p_{\lvert P \rvert} \lvert P \rvert + 
%		                p_{\lvert P \rvert^2} \lvert P \rvert^2 +
%		                p_{\lvert P \rvert^3} \lvert P \rvert^3)
%\end{split}
%\end{equation*}
%where $P$ denotes the set of statements in an input method. The last step is derived based on an overly conservative approximation that Algorithm~\ref{alg:findregion} will always traverse the maximum number of subsets to find the minimal subset \eg, $\lvert P \rvert$ for size of 1, $\lvert P \rvert * (\lvert P \rvert - 1)$ for size of 2 and $\lvert P \rvert * (\lvert P \rvert - 1) * (\lvert P \rvert - 2)$ for size of 3. 
%
%Assigning the probability according to the distribution of over eight hundred thousand test methods in the three datasets for code2seq (all other evaluated models have similar distributions).
%%Java-small, Java-med, and Java-large:
%\begin{equation} \label{eq:eq3}
%\begin{split}
%%t_{ave} & < t_{one} (0.831 \lvert P \rvert + 
%%0.157 \lvert P \rvert^2 + 0.012 \lvert P \rvert^3)
%t_{ave} & < t_{one} (0.406 \lvert P \rvert + 
%0.589 \lvert P \rvert^2 + 0.005 \lvert P \rvert^3)
%\end{split}
%\end{equation}
%
%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=1.25]
%	\begin{axis}[
%	xmax=80,xmin=1,
%	ymin=0,ymax=7000,
%	xlabel=\emph{Number of Statements},ylabel=\emph{Running Time (ms)},
%	xtick={1,10,20,...,80},
%	ytick={0,1000,2000,...,7000},
%	%	x dir=reverse,
%	label style={font=\scriptsize},%added by wy
%	tick label style={font=\tiny} ,
%	legend style={
%		at={(0.01,.99)},
%		anchor=north west,
%		font=\bfseries\scriptsize,
%	}
%	% xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
%	]
%	\addplot+ [mark=triangle*,mark size=1.8pt,every mark/.append style={}] coordinates{(1, 1) (5, 25) (10, 100) (15,225) (20, 400) (25, 625) (30, 900) (35,1225) (40,1600) (45, 2025) (50, 2500) (55, 3025) (60, 3600) (65, 4225) (70, 4900) (75, 5625) (80, 6400)};   
%	%\addplot+ [mark=square*,mark size=1.5pt,every mark/.append style={}] coordinates{(1, 0.831) (5, 8.015) (10,31.08) (15,78.195) (20, 158.36) (25, 280.575) (30, 453.84) (35,687.155) (40,989.52) (45, 1369.935) (50, 1837.4) (55, 2400.915) (60, 3069.48) (65, 3852.095) (70, 4757.76) (75, 5795.475) (80, 6974.24)};
%	\addplot+ [mark=square*,mark size=1.5pt,every mark/.append style={}] coordinates{(1, 1) (5, 17.38) (10, 67.96) (15, 155.49) (20, 283.72) (25, 456.4) (30, 677.28) (35, 950.11) (40, 1278.64) (45, 1666.62) (50, 2117.8) (55, 2635.93) (60, 3224.76) (65, 3888.04) (70, 4629.52) (75, 5452.95) (80, 6362.08)};
%														
%	
%	\legend{Quadratic time algorithm, Average-case complexity}
%	\end{axis}
%	\end{tikzpicture}
%	\caption{Average-case complexity of Algorithm~\ref{alg:findregion}.}
%	\label{fig:time}
%\end{figure}
%
%Figure~\ref{fig:time} plots the upper bound of $t_{ave}$ (\ie, the right side of Equation~\ref{eq:eq3}) \wrt the number of statements in a method assuming $t_{one}$ takes one millisecond.
%We adopt the interquartile range to exclude outliers in the three datasets based on the number of statements in a method. This measure determines the cut-off value to be around 80, which covers more than 99\% of the methods in the three datasets. 
%Clearly, Algorithm~\ref{alg:findregion} runs even faster than a quadratic algorithm with the same constant factor $t_{one}$ most of the time. Given the scale and generality of the experimented inputs, we believe the average-case complexity would apply to any arbitrary set of methods for the four evaluated models.

\subsection{Mutate}

In the \textit{Mutate} step, we aim to pinpoint the defining features within the minimal code fragment discovered by the \textit{Reduce} step. 

\begin{algorithm}[tbp]
	\algnewcommand\Pd{prediction\xspace}
	\algnewcommand\Ml{model\xspace}
	\algnewcommand\OMT{method\xspace}
	\algnewcommand\K{i\xspace}	
	\algnewcommand\Mn{met.name\xspace}		
	\algnewcommand\Me{met\xspace}
	\algnewcommand\Mt{met\_ast\xspace}
	\algnewcommand\Md{mini\_met\xspace}
	\algnewcommand\Ma{mini\_ast\xspace}
	\algnewcommand\Fe{features\xspace}
	\algnewcommand\Ne{node\xspace}
	\algnewcommand\Tn{target\_node\xspace}
	\algnewcommand\Fg{flag\xspace}
	\algnewcommand\Nt{node.children\xspace}
	\algnewcommand\Nz{node.children.size\xspace}	
	\algnewcommand\Ni{node.children[i]\xspace}	
	\algnewcommand\Na{node.children[node.value[1]]\xspace}	
	\algnewcommand\Nv{node.value\xspace}
	\algnewcommand\No{node.value[0]\xspace}	
	\algnewcommand\Nn{node.value[1]\xspace}	
	\algnewcommand\Ve{value\xspace}
	\algnewcommand\Pl{oov\xspace}		
	\algnewcommand\Rt{root\xspace}
	\algnewcommand\Ry{root.copy\xspace}	
	\algnewcommand\Ss{s\xspace}
	\algnewcommand\Ch{child\xspace}
	\algnewcommand\Cs{replace\xspace}
	\algnewcommand\Rv{replace.value\xspace}
	\algnewcommand\Cv{child.value\xspace}
	\algnewcommand\Cz{child.value[0]\xspace}	
	\algnewcommand\Co{count\xspace}
	\algnewcommand\Ps{pos\xspace}	
	\algnewcommand\Vo{oov\xspace}	
	\algnewcommand\NB{node\_bck\xspace}	
	\algnewcommand\FMN{MutateNode\xspace}	
	\algnewcommand\FDN{DeleteNode\xspace}	
	\algnewcommand\FIN{InheritNode\xspace}	
	\algnewcommand\NewV{new\_value\xspace}	
	\algnewcommand\Ncv{node.children[0].value\xspace}	
	\algnewcommand\IV{IsValid\xspace}	
	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}
	
	\caption{Find the defining features in the minimal code fragment.}
	\label{alg:keyfea}
	\begin{algorithmic}[1]
		%\Statex \textbf{define} PASS True
		%\Statex \textbf{define} FAIL False 
		\item[]
		
		\Procedure{FindFeatures}{$\Md, \OMT, \Ml$}
		\State \Rt $\gets$ \textit{Parse}\!\:\!\:(\Md).\Rt 		%\Comment{extracting AST from the minimal method \textit{\Md}}
		\State \Call{Mutate}{\Rt, \Rt, \OMT, \Ml} \Comment{{\Md} is the minimal fragment of {\OMT}}
		\State	\Return{\Rt}
		\EndProcedure
		
		\item[]
		
		\Function{Mutate}{$\Ne, \Rt, \Me, \Ml$}
		\Foreach{\Ch $\in$ \Nt} %\Comment{processing all children nodes first}
		\State \Call{Mutate}{\Ch, \Rt, \Me, \Ml} 
		\EndForeach
		
		\State \Co $\gets$ \Nz %\Comment{counting \# of children nodes}
		\State \NB $\gets$ \Ne \Comment{backing up {node}}
		
		\If{count == 0} \label{alg:mut:count0beg}
		\If{\textbf{not} \Call{\FDN}{\Ne, \NB, \Rt, \Me, \Ml}}  \label{line:wrap1}\Comment{removing {node} }
		\State \Call{\FMN}{\Ne, \NB, \Rt, \Me, \Ml}\label{line:wrap2}   \Comment{if fails, mutating {node}}
		
		\EndIf \label{alg:mut:count0end}
		%\ElsIf{count == 1} \label{alg:mut:count1beg} \Comment{if \textit{node} has only one child}  
		%	\State \Call{\FIN}{\Ne, \NB, \Rt, \Me, \Ml} \Comment{replacing \textit{node} with its child}
		\EndIf  \label{alg:mut:count1end}
		
		\EndFunction
		
		
		%\Function{Mutate}{$\Ne, \Rt, \Me, \Ml$}
		%\Foreach{\Ch $\in$ \Nt}
		%    \State \Call{Mutate}{\Ch, \Rt, \Me, \Ml}
		%\EndForeach
		%
		%\LineComment{counting \# of children nodes that can't be replaced with random tokens}
		%\State \Co $\gets 0$; \Ps $\gets -1$
		%\For{\K $\gets 0$ \textbf{to} \Nz}
		%	\State \Ch $\gets$ \Ni
		%	\If{\Cz $\neq$ \Pl}  \Comment{if the current node is not a random token}
		%		\State\Co\!++; \Ps $\gets \K$
		%	\EndIf
		%\EndFor
		%\LineComment{two conditions to be considered when processing a node: }
		%\If{isTokenizable\:\!\:\!$($\!\!\:\Ne\!\!\:\!$)$} \Comment{(1) if the node can be replaced with a random token}
		%
		%	\If{\Co $= 0$ \textbf{or} \Co $= 1$ \label{line:iftwo}}  \Comment{then maximum one necessary child allowed}
		%		\State \Call{Wrapper}{\Ne, \Ps, \Rt, \Me, \Ml}\label{line:wrap1}
		%	\EndIf
		%\ElsIf{isRemovable\:\!\:\!$($\!\!\:\Ne\!\!\:\!$)$} \Comment{(2) if the node can only be removed}
		%	\If{\Co $= 0$\label{line:ifone}} \Comment{then no necessary child is allowed}
		%		\State \Call{Wrapper}{\Ne, $\infty$, \Rt, \Me, \Ml}\label{line:wrap2}
		%	\EndIf
		%\EndIf
		%\EndFunction
		\item[]
		
		\Function{\FDN}{$\Ne, \NB, \Rt, \Me, \Ml$} \label{alg:mut:removebeg}
		\State \Ne $\gets$ \textit{Delete}\! (\Ne) %\Comment{removing the current node}  
		\State \Return{\Call{\IV}{\Ne, \NB, \Rt, \Me, \Ml}} 
		\EndFunction \label{alg:mut:removeend}
		
		\item[]
		
		\Function{\FMN}{$\Ne, \NB, \Rt, \Me, \Ml$} \label{alg:mut:mutatebeg}
%        \LineComment{\hspace{\algorithmicindent} \(\triangleright\)  mutating \textit{node} into one with out-of-vocabulary value.}
		\State \Ne $\gets$ \textit{Replace}\! (\Ne, oov) \Comment{mutating {node} into \texttt{oov} node}
		\State \Return{\Call{\IV}{\Ne, \NB, \Rt, \Me, \Ml}}
		\EndFunction \label{alg:mut:mutateend}
		
		%\item[]
		
		%\Function{\FIN}{$\Ne, \NB, \Rt, \Me, \Ml$} \label{alg:mut:inheritbeg}
		%\State \Ne $\gets$ \textit{Replace}\! (\Ne, node.children[0]) \Comment{replacing \textit{node} with its only child node}
		%%\State \Ne $\gets$ \textit{Delete}\! (node.children[0]) \Comment{removing the child node}
		%\State \Return{\Call{\IV}{\Ne, \NB, \Rt, \Me, \Ml}}
		%\EndFunction \label{alg:mut:inheritend}
		
		\item[]
		
		
		\Function{\IV}{$\Ne, \NB, \Rt, \Me, \Ml$} \label{alg:mut:consbeg}
		\State suff\_mth, nec\_mth $\gets$ \textit{ReconstructByNode}\! (\Rt, \Ne, \Me)\label{line:rstnode}
		%\If{\textbf{not} \textit{Verify}({\Rt, \Me, \Ml})} }
		\If{\textit{Verify}\! ({suff\_mth, nec\_mth, \Ml}) \label{line:notverify}} %\Comment{if  both \textit{sufficient} and \textit{necessary} are satisfied}
		\State	\Return{True}
		\EndIf
		\State \Ne $\gets$ \textit{RestoreNode}\! (\NB)\Comment{reverting to the backup node}
		\State \Return{False} 
		\EndFunction \label{alg:mut:consend}
		\item[]
		%\Function{Verify}{$\Rt, \Me, \Ml$}
		%\State \Ma $\gets$ \Call{Refresh}{\Ry}\;\label{line:ref}				
		%			
		%\State \Mt $\gets$ \Call{Parse}{\Me}
		%\State \Pd $\gets$ \Ml.\textit{Predict}(\Call{Serialize}{\Call{Compress}{\Mt\!$\setminus$\! \Ma}})\;\label{line:remkey}
		%\If{\Pd $\neq$ \Mn} 									 
		%	\State \!\!\Pd $\gets$ \Ml.\textit{Predict}(\Call{Serialize}{\textit{Deco}\!\:\!\:(\Call{Compress}{\Ry})})\;\label{line:suff}
		%	\If{\Pd $=$ \Mn} 
		%		\State \Return{\textit{True}}
		%	\EndIf
		%	\State  \Return{\textit{False}}	
		%\EndIf
		%\EndFunction
		
		%\algstore{myalg}
	\end{algorithmic}
\end{algorithm}

%Technically, we identify the defining features from the minimal method's AST. \wyc{The following is modified}
%Unlike the \textit{Reduce} step, we do not traverse the sets of nodes in the ascending order of the size due to the following two reasons: (1) the set of nodes that comprises the defining features may not be small, so the style of search adopted by the \textit{Reduce} step is likely to be highly inefficient for the \textit{Mutate} step; (2) combining tokens from the minimal features is inaccurate because it discards the actual tree structure of the program's AST. For example, \texttt{foo.bar(arg)} consists of three tokens \texttt{foo}, \texttt{bar}, \texttt{arg}. One combination of two tokens is \texttt{foo(arg);}, but models may use the field access expression on the object \texttt{foo} (without the name of the field \texttt{bar}) as the defining feature. 
%Therefore, in the \textit{Mutate} step, we mix the mutation and deletion operation from the minimal method's AST to pinpoint both the explicit and implicit fine-grained features.
%
%%For the sake of the precision, 
%\ke{Yu, the key is both the algorithm and the text need to clearly reflect that we first delete and then mutate. Give details of each step, and WHY we do what we do. \wyc{I explain the reason in the last paragraph. I explain my revised algorithm in the next paragraph.}}

Algorithm~\ref{alg:keyfea} gives the details. At a high-level, we perform a postorder traversal on the AST of the minimal statements. For each node operation, we consider the following two cases. If a node does not have any child node, then we first try deleting the node (line~\ref{line:wrap1}). If the resultant program no longer satisfies both the \textit{sufficient} and \textit{necessary} requirement, we will mutate the node into one with an out-of-vocabulary value (line~\ref{line:wrap2}). As explained in Section~\ref{sec:over}, the reason we attempt the deletion operation prior to the mutation operation is that even when an expression can not be further reduced, we may only need to retain its syntactic structure without the specific identifier names. 
%the actual features models use for prediction. 
If a node has children nodes,
% the current node will inherit from its child, and the child node will be removed as a result (lines~\ref{alg:mut:count1beg} to \ref{alg:mut:count1end}). Lastly, if a node has more than one node, 
the parent node will be kept intact to preserve the status of its children. Note that whenever we attempt to delete a node, we may delete addition nodes (\ie, the minimal set of nodes required) just to ensure the syntactic validity of the resultant programs. If the node happens to be irremovable, we simply skip the deletion operation. The same strategy also applies to mutation operations.

%Below we will give a step-by-step illustration for reducing the statement \texttt{return cond1 || cond2}. \ke{Yu, describe the workflow CLEARLY with a figure!!!! The following is STILL NOT clear}.
%
%
%\begin{figure}[htbp]
%\begin{tikzpicture}[font=\small]
%
%\Tree [.\node[ellipse, draw](a) {Root}; 
%          [.\node[ellipse, draw] (c) {BlockStmt};
%            [.\node[ellipse, draw] (d) {ReturnStmt}; 
%              [.\node[ellipse, draw] (e) {BinaryExpr: \texttt{||}}; 
%                [.\node[rectangle, draw] (f) {cond1}; ] 
%                [.\node[rectangle, draw] (g) {cond2}; ] 
%              ]
%             ]
%          ]
%          %[.\node (b) {\dots}; ] 
%      ] 
% 
% 
%\begin{scope}[xshift=2.75cm]
%\Tree [.\node[ellipse, draw](da) {Root}; 
%          [.\node[ellipse, draw] (dc) {BlockStmt};
%            [.\node[ellipse, draw] (dd) {ReturnStmt}; 
%                [.\node[rectangle, draw] (df) {cond2}; ] 
%             ]
%          ]
%          %[.\node (bb) {\dots}; ] 
%      ] 
%\end{scope}
%
%\begin{scope}[xshift=5.5cm]
%\Tree [.\node[ellipse, draw](aa) {Root}; 
%          [.\node[ellipse, draw] (ac) {BlockStmt};
%            [.\node[ellipse, draw] (ad) {ReturnStmt}; 
%              [.\node[ellipse, draw] (ae) {BinaryExpr: \texttt{||}}; 
%                [.\node[rectangle, draw] (af) {\phantom{d}oov\phantom{d}}; ] 
%                [.\node[rectangle, draw] (ag) {cond2}; ] 
%              ]
%             ]
%          ]
%          %[.\node (ab) {\dots}; ] 
%      ] 
% \end{scope}
%
%\begin{scope}[xshift=8.25cm]
%\Tree [.\node[ellipse, draw](ba) {Root}; 
%          [.\node[ellipse, draw] (bc) {BlockStmt};
%            [.\node[ellipse, draw] (bd) {ReturnStmt}; 
%                [.\node[rectangle, draw] (bf) {cond1}; ] 
%             ]
%          ]
%          %[.\node (bb) {\dots}; ] 
%      ] 
%\end{scope}
%
%\begin{scope}[xshift=11cm]
%		\Tree [.\node[ellipse, draw](ca) {Root}; 
%          [.\node[ellipse, draw] (cc) {BlockStmt};
%            [.\node[rectangle, draw] (cd) {ExprStmt}; 
%              [
%              .\node[rectangle, draw] (cd) {cond1};
%              ]
%             ]
%          ]
%           %[.\node (cb) {\dots}; ] 
%     ]  
%\end{scope}
%
%
% 
%\node[
%	below=4.2cm of a] (h) {  
%	\texttt{return cond1||cond2;}
%}; 
%\node[
%	above=1mm of a] (h) {  	
%	\textbf{\scriptsize{\textit{Step} \circled{1}}}
% }; 
% 
%\node[
%	below=4.2cm of da] (h) {  
%	\texttt{return cond2;}
%}; 
%\node[
%	above=1mm of da] (h) {  	
%	\textbf{\scriptsize{\textit{Step} \circled{2}}}
% }; 
% 
% \node[
% 	below=4.2cm of aa] (i) {  
%	\texttt{return oov||cond2;}
%}; 
%\node[
% 	above=1mm of aa] (i) {  
% 	\textbf{\scriptsize{\textit{Step} \circled{3}}}
%}; 
%
%\node[
% 	below=4.2cm of ba] (j) {  
%    \texttt{return  cond1;}
% }; 
%\node[
% 	above=1mm of ba] (j) {        
%	\textbf{\scriptsize{\textit{Step} \circled{4}}}
% }; 
% 
% 
%\node[
% 	below=4.2cm of ca] (j) {  
%      \texttt{cond1;}
% }; 
%\node[
% 	above=1mm of ca] (j) {        
%	\textbf{\scriptsize{\textit{Step} \circled{5}}}
% }; 
% 
%\path (a) -- node {$\stackrel{}{\implies}$} (da);
%\path (da) -- node {$\stackrel{}{\implies}$} (aa);
%\path (aa) -- node{$\stackrel{}{\implies}$} (ba);
%\path (ba) -- node{$\stackrel{}{\implies}$} (ca);
%
%\end{tikzpicture}
%\caption{Deleting, mutating and inheriting nodes in the AST of \texttt{return cond1 || cond2;} }
%\label{fig:astexp}
%\end{figure}
%
%Figure~\ref{fig:astexp} gives an example to show the procedure when processing \texttt{return cond1||cond2;}. The ASTs in the figure omit other structures such as the method type for the sake of simplicity. We first try to delete the node of \texttt{cond1}. But directly deleting the node results in \texttt{return ||cond2;}, which is an invalid AST, so we greedily delete its parent nodes to construct a valid AST. In this example, we delete \texttt{cond1||}, resulting in \texttt{return cond2;} (\textit{Step }\textbf{\circled{2}}). If \texttt{return cond2;} fails to satisfy both \textit{sufficient} and \textit{necessary} requirements, then we try to mutate \texttt{cond2} to \texttt{oov} (\textit{Step }\textbf{\circled{3}}). Assume \texttt{return oov||cond2;} still fails to meet the two requirements, we move on to the node of \texttt{||}, since deleting \texttt{||} also leads to an invalid AST (\ie, \texttt{return cond1 cond2;}) , we keep applying greedily deletion but avoid deleting duplicated tokens, which means we delete \texttt{||cond2}, resulting in \texttt{return cond1;}(\textit{Step }\textbf{\circled{4}}). Then, assume the new method satisfies both requirements but \texttt{return;}, constructed by deleting \texttt{cond1} in \texttt{return cond1;}, does not. In this case, we will process the node of \texttt{return} by inheriting node \texttt{ReturnStmt} from \texttt{cond2}, resulting in \texttt{cond2;}(\textit{Step }\textbf{\circled{5}}), which satisfies both requirements and is the final output of the \textit{Mutate} step. \wyc{I add ExprStmt in step 5 because \texttt{cond1;} is not a kind of block statement.}

%For example, assume we have removed token \texttt{cond1} in \texttt{return cond1 || cond2;}, resulting in \texttt{return cond2;}, then when processing the node of \texttt{return}, we will inherit node \texttt{return} from \texttt{cond2}, resulting in \texttt{cond2;}. 

%For functions explicitly defined in Algorithm~\ref{alg:keyfea}, \textit{ConstructAndVerify} constructs new methods based on a new node, verifies the \textit{sufficient} and \textit{necessary} requirements,  reverts the new node back to its original node if the verification fails, and returns the result of the verification (lines~\ref{alg:mut:consbeg} to \ref{alg:mut:consend}). 
%\textit{DeleteNode} removes \textit{node} from the \textit{root} node and returns the result of \textit{ConstructAndVerify} (lines~\ref{alg:mut:removebeg} to \ref{alg:mut:removeend}),
%\textit{MutateNode} replaces  \textit{node} with an  out-of-vocabulary (\textit{oov}) word and returns the result of \textit{ConstructAndVerify} (lines~\ref{alg:mut:mutatebeg} to \ref{alg:mut:mutateend}). 
%\textit{InheritNode} replaces  \textit{node} from its only child node, removes the child node, and returns the result of \textit{ConstructAndVerify} (lines~\ref{alg:mut:inheritbeg} to \ref{alg:mut:inheritend}).  
%Since we only edit the value while mutating (or even deleting) a node, the structure of the minimal method's AST is always preserved, which allows an easier and cleaner \textit{subtraction} operation (\cf Definition~\ref{def:nodes}). At the same time, the actual tree structure is recovered out of the mutated AST in order for the \textit{sufficient} and  \textit{necessary} requirements to be checked against (line~\ref{line:rstnode} and \ref{line:notverify}). 
%\texttt{ReconstructByNode} function solves this problem. The key is to translate the value of each node into a series of tree-edit operations. Note that within the \texttt{Verify} function, tree-edit operations always modify a separate tree copy to preserve the integrity of the mutated AST.
%when we check a method against the \textit{sufficient} or \textit{necessary} requirement, 
% by recursively mutating the parent node whenever a child node has been mutated,
For other functions not explicitly defined in Algorithm~\ref{alg:keyfea}, \texttt{Parse} extracts the AST out of a method, \texttt{Delete} removes a node, \texttt{Replace} replaces  a node with a new node, \texttt{Rec\-onstru\-ctByNode} constructs method \texttt{suff\_mth} for verifying against the \textit{sufficient} requirement and method \texttt{nec\_mth} for verifying against the \textit{necessary} requirement, and finally \textit{RestoreNode} reverts a node back to the saved node.

%\texttt{Serialize} converts an AST back to a method, \texttt{Deco} ensures the construction of syntactically valid methods based on a set of pre-defined rules, and finally \texttt{isTokenizable} /\texttt{isRemovable} returns the mutability/removability of a node.

%\vspace{100pt}



%\begin{algorithm}[!tbp]
%	\SetKwInOut{Input}{input}
%	\SetKwInOut{Output}{output}
%	
%	\DontPrintSemicolon
%	\SetKwProg{myproc}{procedure}{}{}
%	\SetKwFunction{proc}{FindFeatures}
%	\SetKwProg{myfunc}{function}{}{}
%	\SetKwFunction{procc}{Mutate}	
%	\SetKwFunction{proco}{Verify}		
%	\SetKwFunction{prore}{Refresh}		
%	\SetKwFunction{procm}{Compress}		
%	\SetKwFunction{prowr}{Wrapper}		
%	
%	\SetKwData{Pd}{prediction}
%	\SetKwData{Ml}{model}
%	\SetKwData{K}{i}	
%	\SetKwData{Mn}{met.name}		
%	\SetKwData{Me}{met}
%	\SetKwData{Mt}{met\_ast}
%	\SetKwData{Md}{mini\_met}
%	\SetKwData{Ma}{mini\_ast}
%	\SetKwData{Fe}{features}
%	\SetKwData{Ne}{node}
%	\SetKwData{Tn}{target\_node}
%	\SetKwData{Fg}{flag}
%	\SetKwData{Nt}{node.children}
%	\SetKwData{Nz}{node.children.size}	
%	\SetKwData{Ni}{node.children[i]}	
%	\SetKwData{Na}{node.children[node.value[1]]}	
%	\SetKwData{Nv}{node.value}
%	\SetKwData{No}{node.value[0]}	
%	\SetKwData{Nn}{node.value[1]}	
%	\SetKwData{Ve}{value}
%	\SetKwData{Pl}{place\_holder}		
%	\SetKwData{Rt}{root}
%	\SetKwData{Ry}{root.copy}	
%	\SetKwData{Ss}{s}
%	\SetKwData{Ch}{child}
%	\SetKwData{Cs}{replace}
%	\SetKwData{Rv}{replace.value}
%	\SetKwData{Cv}{child.value}
%	\SetKwData{Cz}{child.value[0]}	
%	\SetKwData{Co}{count}
%	\SetKwData{Ps}{pos}	
%	\SetKwData{Vo}{oov}	
%	
%	
%	\SetKw{Break}{break}
%	\SetKw{Not}{not}
%	\SetKw{Or}{or}
%	\SetKw{Ot}{to}
%	
%	\Input{\Md, \Me, \Ml}
%	\Output{\Rt}
%	\myproc{\proc{\Md, \Me, \Ml}}{ 
%		\Begin{			
%			\Rt $\gets$ \textit{Parse}\!\:\!\:(\Md).\Rt \\			
%			\textit{Mutate}\!\:\!\:(\Rt, \Rt, \Me, \Ml)	\\
%			\Return{\Rt}
%		}
%	}
%	
%	%	\tcc{the main procedure of removing redundant nodes from the minimal method's AST}
%	\myfunc{\procc{\Ne, \Rt, \Me, \Ml}}{
%		\Begin{
%			\ForEach{\Ch $\in$ \Nt} {
%				\textit{Mutate}\!\:\!\:(\Ch, \Rt, \Me, \Ml)
%			}
%			\tcc{counting \# of children nodes that can't be replaced with random tokens}
%			\Co $\gets 0$; \Ps $\gets -1$\\
%			\For{\K $\gets 0$ \Ot \Nz}{
%				\Ch $\gets$ \Ni\\
%				\If{\Cz $\neq$ \Pl} {
%					\Co\!++; \Ps $\gets \K$
%				}				
%			}
%			\tcc{two conditions to be considered when processing a node: (1) if the node can be replaced with a random token}
%			\If{isTokenizable\:\!\:\!$($\!\!\:\Ne\!\!\:\!$)$} {
%				\tcp{maximum one necessary child allowed}
%				\If{\Co $= 0$ \Or \Co $= 1$ \label{line:iftwo}} {
%					\textit{Wrapper}(\Ne, \Ps, \Rt, \Me, \Ml)\label{line:wrap1}
%				}				
%			}
%			\tcc{(2) if the node can only be removed}
%			\ElseIf{isRemovable\:\!\:\!$($\!\!\:\Ne\!\!\:\!$)$} {
%				\tcp{no necessary child is allowed}
%				\If{\Co $= 0$\label{line:ifone}} {
%					\textit{Wrapper}(\Ne, $\infty$, \Rt, \Me, \Ml)\label{line:wrap2}
%				}	
%			}
%		}
%	}
%	
%	\myfunc{\prowr{\Ne, \Ps, \Rt, \Me, \Ml}}{
%		\Ve $\gets$ \Nv \\
%		\Nv $\gets$ (\Pl, \Ps) \\
%		
%		\If{\Not Verify\:\!\:\!$($\!\!\:\Rt, \Me, \Ml\!\!\:\!$)$}{
%			\Nv $\gets$ \Ve
%		}		
%	}
%	
%	
%	
%	\myfunc{\proco{\Rt, \Me, \Ml}}{\label{line:44}
%		\Begin{
%			\Ma $\gets$ \textit{Refresh}\! (\Ry)\;\label{line:ref}				
%			
%			\Mt $\gets$ \textit{Parse}\!\:\!\:(\Me) \\
%			\Pd $\gets$ \Ml.\textit{Predict}\! \\\quad\!(\textit{Serialize}\! (\textit{Compress}\!\:\!\:(\Mt\!$\setminus$\! \Ma)))\;\label{line:remkey}
%			\If{\Pd $\neq$ \Mn} {										 
%				\!\!\Pd $\gets$ \Ml.\textit{Predict}\, (\textit{Serialize}\!\:\!\:(\textit{Deco}\!\:\!\:(\textit{Compress}\!\:\!\:(\Ry))))\;\label{line:suff}
%				\If{\Pd $=$ \Mn} {
%					\Return{\textit{True}}
%				}
%			}
%			\Return{\textit{False}}	
%		}
%	}
%	
%	\caption{Find key features in a minimal method. \ke{simplify again fitting it in one page}}
%	\label{alg:keyfea}
%\end{algorithm}

%
%
%\begin{algorithm}[!tbp]
%	\algnewcommand\Pd{prediction\xspace}
%	\algnewcommand\Ml{model\xspace}
%	\algnewcommand\K{i\xspace}	
%	\algnewcommand\Mn{met.name\xspace}		
%	\algnewcommand\Me{met\xspace}
%	\algnewcommand\Mt{met\_ast\xspace}
%	\algnewcommand\Md{mini\_met\xspace}
%	\algnewcommand\Ma{mini\_ast\xspace}
%	\algnewcommand\Fe{features\xspace}
%	\algnewcommand\Ne{node\xspace}
%	\algnewcommand\Tn{target\_node\xspace}
%	\algnewcommand\Fg{flag\xspace}
%	\algnewcommand\Np{node.parent\xspace}
%	\algnewcommand\Nt{node.children\xspace}
%	\algnewcommand\Nz{node.children.size\xspace}	
%	\algnewcommand\Ni{node.children[i]\xspace}	
%	\algnewcommand\Na{node.children[node.value[1]]\xspace}	
%	\algnewcommand\Nv{node.value\xspace}
%	\algnewcommand\No{node.value[0]\xspace}	
%	\algnewcommand\Nn{node.value[1]\xspace}	
%	\algnewcommand\Ve{value\xspace}
%	\algnewcommand\Pl{place\_holder\xspace}		
%	\algnewcommand\Rt{root\xspace}
%	\algnewcommand\Ry{root.copy\xspace}	
%	\algnewcommand\Ss{s\xspace}
%	\algnewcommand\Ch{child\xspace}
%	\algnewcommand\Cs{replace\xspace}
%	\algnewcommand\Rv{replace.value\xspace}
%	\algnewcommand\Cv{child.value\xspace}
%	\algnewcommand\Cz{child.value[0]\xspace}	
%	\algnewcommand\Co{count\xspace}
%	\algnewcommand\Ps{pos\xspace}	
%	\algnewcommand\Vo{oov\xspace}	
%
% \begin{algorithmic}[1]
% \algrestore{myalg}
%
%\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}
%
%\Function{Refresh}{$\Ne$} \Comment{lays the groundwork for \textit{subtraction} operation \wyc{I think the following code is no longer needed}}
%\Foreach{\Ch $\in$ \Nt} 
%	\State \Call{Refresh}{\Ch}
%	\If{\Cz $=$ \Pl} 
%		\State \Nv $\gets$ (\Pl, $-1$)
%		\State \textbf{break}
%	\EndIf	
%\EndForeach
%\State \Return{\Ne}
%\EndFunction
%
%\item[]
%
%\Function{Compress}{$\Ne$} \label{line:comp}
%\Foreach{\Ch $\in$ \Nt} 
%	\State \Call{Compress}{\Ch}
%\EndForeach
%\If{\No $=$ \Pl} \Comment{if node happpens to be unnecessary}
%	\If{\Nn $=$ $\infty$} 
%		%\Comment{if node can only be deleted, delete the subtree rooted at node}
%		\Comment{if node can only be deleted}
%		\State \Np.\textit{remove}\:\!(\Ne) \Comment{deleting the subtree rooted at node}
%	\Else
%		%\Comment{if node has one necessary child, propagate its value to the node}
%			\If{\Nn $\neq -1$} \Comment{if node has one necessary child}
%				\State \Cs $\gets$ \Na \Comment{propagating its value to the node}
%				\State \Nv $\gets$ \Rv 
%			\EndIf
%			\State \Ne.\textit{removeChildren}() \Comment{either case removes all children}
%	\EndIf
%\Else  \Comment{if node happens to be necessary}
%	\Foreach{\Ch $\in$ \Nt} \Comment{only replacing the unnecessary child nodes with out-of-vocabulary tokens}
%		\If{\Cz $=$ \Pl} 
%			\State\Cv $\gets$ (\Vo, $-1$) 
%		\EndIf
%	\EndForeach
%\EndIf
%		
%\State \Return{\Ne}
%\EndFunction
%
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%	
%	\setcounter{AlgoLine}{34}
%	
%	\DontPrintSemicolon
%	\SetKwProg{myfunc}{function}{}{}
%	\SetKwFunction{prore}{Refresh}		
%	\SetKwFunction{procm}{Compress}		
%	
%	\SetKwData{Pd}{prediction}
%	\SetKwData{Ml}{model}
%	\SetKwData{K}{i}	
%	\SetKwData{Mn}{met.name}		
%	\SetKwData{Me}{met}
%	\SetKwData{Mt}{met\_ast}
%	\SetKwData{Md}{mini\_met}
%	\SetKwData{Ma}{mini\_ast}
%	\SetKwData{Fe}{features}
%	\SetKwData{Ne}{node}
%	\SetKwData{Tn}{target\_node}
%	\SetKwData{Fg}{flag}
%	\SetKwData{Np}{node.parent}
%	\SetKwData{Nt}{node.children}
%	\SetKwData{Nz}{node.children.size}	
%	\SetKwData{Ni}{node.children[i]}	
%	\SetKwData{Na}{node.children[node.value[1]]}	
%	\SetKwData{Nv}{node.value}
%	\SetKwData{No}{node.value[0]}	
%	\SetKwData{Nn}{node.value[1]}	
%	\SetKwData{Ve}{value}
%	\SetKwData{Pl}{place\_holder}		
%	\SetKwData{Rt}{root}
%	\SetKwData{Ry}{root.copy}	
%	\SetKwData{Ss}{s}
%	\SetKwData{Ch}{child}
%	\SetKwData{Cs}{replace}
%	\SetKwData{Rv}{replace.value}
%	\SetKwData{Cv}{child.value}
%	\SetKwData{Cz}{child.value[0]}	
%	\SetKwData{Co}{count}
%	\SetKwData{Ps}{pos}	
%	\SetKwData{Vo}{oov}	
%	
%	\SetKw{Break}{break}
%	\SetKw{Not}{not}
%	\SetKw{Or}{or}
%	\SetKw{Ot}{to}	
%	
%	\tcp{lays the groundwork for \textit{subtraction} operation}
%	\myfunc{\prore{\Ne}}{
%		\ForEach{\Ch $\in$ \Nt} {
%			\textit{Refresh}\:\!(\Ch)\\
%			\If{\Cz $=$ \Pl} {
%				\Nv $\gets$ (\Pl, $-1$)\\
%				\Break			
%			}		
%		}
%				
%		\Return{\Ne}
%	}	
%	
%	\myfunc{\procm{\Ne}}{\label{line:comp}
%		\ForEach{\Ch $\in$ \Nt} {
%			\textit{Compress}\:\!(\Ch)
%		}
%		\tcp{if node happpens to be unnecessary}
%		\If{\No $=$ \Pl} {
%			\If{\Nn $=$ $\infty$} {
%				\tcc{if node can only be deleted, delete the subtree rooted at node}
%				\Np.\textit{remove}\:\!(\Ne)
%			}				
%			\Else{
%				\tcc{if node has one necessary child, propagate its value to the node}
%				\If{\Nn $\neq -1$} {
%					\Cs $\gets$ \Na \\				
%					\Nv $\gets$ \Rv
%				}
%				\tcc{either case remove all children}
%				\Ne.\textit{removeChildren}()
%			}
%		}
%		\tcp{if node happens to be necessary}
%		\Else {
%			\tcc{only replacing the unnecessary child nodes with out-of-vocabulary tokens}
%			\ForEach{\Ch $\in$ \Nt} {
%				\If{\Cz $=$ \Pl} {
%					\Cv $\gets$ (\Vo, $-1$) 
%				}
%			}
%		}
%		
%		\Return{\Ne}
%	}		
%\end{algorithm}

%
%%\vspace{-4pt}
%\begin{definition}(\textit{\textit{Subtraction} of Trees})\label{def:nodes}
%	Let $T$ be the AST of an input method. 
%	Let $\tilde{T}$ be the AST of the minimal method with a set of statements $B$ as the body (discovered by Algorithm~\ref{alg:findregion}). 	
%	Suppose $\tilde{T}$ is transformed to $\bar{T}$ via the mutation operation (specified in Algorithm~\ref{alg:keyfea}). $T \setminus \bar{T}$ is defined as (1) subtracting the subtree $T_{return}$ in $T$ from the subtree $\bar{T}_{return}$ in $\bar{T}$, denoted by $T_{return}\oplus\bar{T}_{return}$ (Definition~\ref{def:trees}), where $T_{return}$ denotes the AST of the return type of the input method, and $\bar{T}_{return}$ denotes the AST of the return type of the mutated method; (2) $T_{paralist}\oplus\bar{T}_{paralist}$ where $T_{paralist}$ denotes the AST of the parameter list of the input method, and $\bar{T}_{paralist}$ denotes the AST of the parameter list of the mutated method; (3) 
%	$\forall S \in B \, T_{S}\oplus\bar{T}_{S}$ where $T_{S}$ denotes the AST of the statement $S$ in the input method, and $\bar{T}_{S}$ denotes the AST of the same statement in the mutated method.
%\end{definition}
%%\vspace{-8pt}
%
%\begin{definition}(\textit{Subtraction Operator})\label{def:trees}	
%	Let $T_1$ be an AST. Let $T_2$ be another AST. $T_{1}\oplus\bar{T}_{2}$ updates the value of each node in $T_{1}$ as follows: (1) if the value of a node in $T_1$, $v_1.\mathit{value}$, equals to the value of the \textit{twin} node in $T_2$, then $v_1.\mathit{value}$ will be updated to \textit{placeholder}. A node in $T_2$ is a \textit{twin} of another node in $T_1$ if the two nodes are overlapped when $T_1$ and $T_2$ are overlaid; (2) if $v_1.\mathit{value}$ differs from the value of the twin node in $T_2$, then it's only possible that the value of the twin node is \textit{placeholder} in which case $v_1$ maintains its value.
%\end{definition}

\vspace*{3pt}
\noindent
\textbf{\textit{Minimality}}\, Obviously, the result of Algorithm~\ref{alg:keyfea} may not satisfy the \textit{minimality} requirement in Definition~\ref{def:keyfea}. In principle, it satisfies the \textit{1-tree-minimality}~\cite{HDD} property because no node can be further removed from the AST of the defining features. On the other hand, the style of search adopted in \textit{Reduce} also can not guarantee the global minimality of its outcome because the defining features may exist in a non-minimal code fragment that \textit{Reduce} can not find. This is the reason that we only consider \textit{1-tree-minimality} in the \textit{Mutate} step, especially given that (1) the size of the defining features is already small, thus the explanations to be generated will be informative to end users; (2) the current algorithm is highly efficient.


% To achieve the global minimality, we further manipulate the AST that Algorithm~\ref{alg:keyfea} returns. In particular, we mutate each subset of its terminals nodes to generate new ASTs, and then check their validity against the \textit{sufficient} and \textit{necessary} requirements. Although this approach yields an exponential time algorithm, the performance is reasonable in practice (\cf Section~\ref{subsec:effic}). 
%Since Algorithm~\ref{alg:keyfea} performs a linear traversal of the input AST, it has a complexity $O(n)$ where $n$ is the number of the nodes in the tree. Given the dominance of \textit{Reduce} in terms of the time 

\vspace*{3pt}
\noindent
\textbf{\textit{Time Complexity}}\, Since Algorithm~\ref{alg:keyfea} performs a linear traversal on the AST of the input program, it has a complexity $O(n)$ where $n$ is the number of the nodes in the tree. Given the dominance of \textit{Reduce} in terms of the time complexity, our method --- \textit{Reduce} and \textit{Mutate} --- runs in exponential time in theory and quadratic time in practice. 




%At this point, we have found the defining features for an input method since they satisfy all requirements --- \textit{sufficient}, \textit{necessary}, and \textit{minimal} --- in Definition~\ref{def:keyfea}.
%
%Move to Appendix B


%\subsection{An Example Use of The Revealed Features}
%\label{subsec:exa}
%
%We utilize the revealed features code summarization models use to explain their predictions. The idea is as follows. Given a Model $M$, and a program $P$ from $M$'s test set for which $M$ predicts $L$. First, we discover the key features $M$ uses to predict $L$; Second, we do the same thing for all programs in $M$'s training set with the label $L$. Note that in a generative setting (\eg, code2seq, sequence GNN) where training set might not contain a method of label $L$, we consider all methods whose name is a subset of the words in $L$. Finally, we rank these training programs based on the distance between their and $P$'s revealed features. Our rationale is to find the training programs from which models extracted the key features at the first place. Thus, our method explains the root cause of a prediction rather than interprets the internal state of models.   






